Predicate Logic as a Modelling Language: The IDP System

With the technology of the time, Kowalski's seminal 1974 paper {\em Predicate Logic as a Programming Language} was a breakthrough for the use of logic in computer science. It introduced two fundamental ideas: on the declarative side, the use of the Horn clause logic fragment of classical logic, which was soon extended with negation as failure, on the procedural side the procedural interpretation which made it possible to write algorithms in the formalism. Since then, strong progress was made both on the declarative understanding of the logic programming formalism and in automated reasoning technologies, particularly in SAT solving, Constraint Programming and Answer Set Programming. This has paved the way for the development of an extension of logic programming that embodies a more pure view of logic as a modelling language and its role for problem solving. In this paper, we present the \idp language and system. The language is essentially classical logic extended with one of logic programmings most important contributions to knowledge representation: the representation of complex definitions as rule sets under well-founded semantics. The system is a knowledge base system: a system in which complex declarative information is stored in a knowledge base which can be used to solve different computational problems by applying multiple forms of inference. In this view, theories are declarative modellings, bags of information, descriptions of possible states of affairs. They are neither procedures nor descriptions of computational problems. As such, the \idp language and system preserve the fundamental idea of a declarative reading of logic programs, while they break with the fundamental idea of the procedural interpretation of logic programs.

==> 3c-architecture.tex <==
\section{Inferences and system architecture}\label{sec:architecture}
%Inferences are the workhorse of reasoning in any \KBS, so it is crucial they are state-of-the-art.
In this section, we discuss the architecture and the inference methods of the \idp system.


\subsection{Main Inferences}
\maurice{TO BE COVERED BY THE PROCEDURE SUBSECTION?}

The \idp system supports a range of functionalities to solve various inference and other logic-related tasks.
%
Below, we specify a task through its input arguments $i_1, \ldots, i_n$, a precondition $Pre(i_1,\dots,i_n)$, output arguments $o_1, \ldots, o_m$, and a postcondition $Post(i_1, \ldots, i_n, o_1, \ldots, o_m)$. This specifies a task as a partial (potentially non-deterministic) function from a space of input values to a space of output values. An \emph{inference} task is a task that has logic objects (logic components, symbols, domain elements, \ldots) as input and output and where the pre- and postcondition depend on semantic properties of these (logically equivalent input has logically equivalent output).
%
For example, the normalization of a formula is considered a task, but not an inference task: an input formula \f is transformed into a logically equivalent formula $\psi$.
%
In the following, we discuss the inference tasks currently supported by \idp.
\todo{rvwr4 Why isn't normalization of a formula considered an inference
task?  It seems to satisfy your def'n?
}
%The \idp system supports a range of functionalities to solve computational tasks.
%We define a computational task as a pattern consisting of a input arguments $i_1, \ldots, i_n$, that satisfy some precondition $Pre$, and output arguments $o_1, \ldots, o_m$, that satisfy some postcondition $Post(i_1, \ldots, i_n, o_1, \ldots, o_m)$.
%Among computational tasks, we distinguish \emph{inference} tasks (inferences), that take only logic objects as in- and output, such as theories or structures, and where the pre- and postcondition depends on semantic properties.
%Computational tasks consist for example of procedures to normalize formulas, whereas querying and deduction are considered inferences.
%As a consequence, inferences 
%We define inference  
%We distinguish general computational , from specific tasks such as normalization of formulas to inference tasks that solve general problems and have logical objects as input and output. 
%We define an \emph{inference} (task) as a computational task that solves a ``general'' problem and has takes a set of logical objects as input and output, such that some relation between input and output is satisfied (given restrictions on the input).

\textbf{Query inference} takes as input a structure \I and a set expression $\{x \mid \f\}$ over a vocabulary $V$ and returns the set $\{x \mid \f\}^\I$.
The formula \f can only contain symbols that are two-valued in \I.
% However, for any symbol $P(\TTT)$ in a vocabulary $V$, $V$ also
% contains two ``derived'' symbols $P_{ct}(\TTT)$ and $P_{cf}(\TTT)$.
% \todo{rvwr4 Why don't you use your object syntax (in Querying Structures with
% sets) instead of base syntax in definitions?  This is a system paper,
% no?  And what is the object syntax for $P_ct$ and $P_cf$ (the predicate
% name with $_ct$ (or $_cf$) suffix?  Should be clarified.)
% }
% In any structure \I over $V$, $P_{ct}$ and $P_{cf}$ are interpreted in \I as the set of all tuples of domain elements for which $P$ is true, respectively false, in \I (and similarly for functions, which are interpreted over their graph).
\bart{Heb hier een stuk weggelaten over $P_{ct}$ en $P_{cf}$ symbolen die tweewaardig kunnen zijn (zie latex in commentaar). We supporteren momenteel geen dergelijke queries.}
Querying is implemented by transforming the set expression into an extended First-Order Binary Decision Diagram and afterwards querying the BDD over \I, as described in~\mycite{GroundingWithBounds}.

\textbf{Model expansion} takes as input a partial structure $\I_{in}$ and an \fodotidp theory \theory, and produces models \I of \theory that expand $\I_{in}$.
\textbf{Optimization inference} takes also a term $t$ as input, and produces models that have a minimal value for $t$.
Both inference tasks are discussed in more detail in Section \ref{sec:mx}.
\textbf{Model checking} is a special case of model expansion with \I a two-valued structure interpreting $voc(\theory)$; it is implemented through model expansion.

\textbf{Propagation} takes as input a theory \theory and a partial structure \I, returning a more precise partial structure $\I_{out}$ that approximates all models of \theory that are expansions of \I~\cite{acm/wittocx}. Equivalently, propagation deduces ground literals that hold in all models of \theory that expand \I. The system provides a complete propagation system (co-NP complete \bart{dit geloof ik niet. Na overleg met Ingmar lijkt het eerder $\Delta^P_2$-hard}) and a sound but incomplete polynomial algorithm based on a lifted form of unit propagation. 
The latter proved very useful for building interactive knowledge-based configuration systems~\cite{ppdp/VlaeminckVD09}. 

\textbf{Deduction} takes as input an \foidp theory \theory and an FO theory $\theory_{FO}$ and returns true if $\theory \models \theory_{FO}$. It is implemented by translating \theory into a (weaker) \FO theory $\theory_0$ and calling the theorem prover Spass~\cite{cade/WeidenbachDFKSW09} to check whether $\theory_0 \models \theory_{FO}$.

\textbf{\D-model expansion} takes as input a definition \D and a structure $\I_{in}$, interpreting all parameters of \D, and returns the unique model \I that expands $\I_{in}$. This task is an instance of model expansion, but is solved in \idp using different technology. The close relationship between definitions and logic programs under the well-founded semantics is exploited to translate \D and $\I_{in}$ into a tabled Prolog program, after which XSB is used to compute \I.
Taking an extra formula \f as input, with free variables \xxx, the same approach is used to solve the query \f with respect to \D and $\I_{in}$ in a goal-oriented way~\cite{tplp/Jansen13}.

\textbf{Symmetry detection} takes as input a theory \theory and a partial structure \I and returns \emph{symmetries} over \theory and \I~\cite{ictai/DevriendtBMDD12}.
A symmetry is a function, say $f$, mapping structures to structures, such that, for any two-valued expansion $J$ of \I, $J \models \theory$ iff $f(J) \models \theory$.

\todo{rvwr4 I'm wondering about the treatment of types in reasoning, say in model
generation.  Your structures contain definitions of types; it would
seem reasonable for a user to expect model generation to generate
meanings for types.  I presume you don't do that, since that would be
quite open-ended.  You allow types to be predicates as well, so that
would imply (to me) that their meanings must be included in model
generation.  You say (somewhere, I think) that types can all be
eliminated in syntactic processing, but with them being allowed as
predicates, I don't see quite how you can guarantee that, without
severe restrictions on their use.  What am I not understanding?
}

In addition to inferences, the system provides a large number of smaller-scale functionalities.
Examples are (model-preserving) normalization procedures, that take a theory \theory and (optionally) a structure \I and transform \theory into a theory satisfying certain properties.
Below, an overview is given of a well-known subset of the normalization procedures provided by \idp.
\begin{description}
  \item[flatten(\theory)] puts disjunction and conjunctions in left-associative form.
  \item[simplify(\theory,\I)] replaces terms and formulas known in \I by their interpretation.
  \item[push-negations(\theory)] puts a theory in negation normal form.
  \item[push-quantifications(\theory)] moves quantifications down if the associated variable does not occur in all subformulas. 
  \item[shared-formula(\theory)] replaces terms and formulas that occur multiple times in \theory (possibly with different variable substitutions), by a new symbol, defined by that term or formula.
  \item[nest-variables(\theory)] uses atoms $x=t$, with $x$ a variable and $t$ a term, to replace $x$ by $t$ wherever allowed, possibly eliminating $x=t$ itself.
  \item[ground(\theory,\I)] transform \theory into a ground theory $\theory_g$ such that models of $\theory_g$ can be mapped one-to-one to models of \theory expanding \I. The ground theory can be transformed into different language formats, through the option \il{stdoptions.language}, such as CNF (Clausal Normal Form), ECNF (the native format of \minisatid) or ground \ASP.
\end{description}

In addition to \fodotidp inferences, more domain-specific inferences are provided.
One example is \text{unsat-debugging}: given a theory \theory and structure \I, $\I \not\models \theory$, find a minimal subset of \theory that is unsatisfiable in \I.
Unsat-debugging is a great aid for users to help pinpoint modelling errors.
Through reuse of the above-mentioned inferences and functionality, it took minimal time to implement in \idp.


\subsection{Internal representation.}
\maurice{DROP??}

The system offers the language \fodotidp to the user, but internally, a more manageable representation is necessary. The main representation closely follows the structure of the \foidaggpf language: each component of the parse-tree is stored as a separate object with pointers to its children. E.g., a \emph{theory}-object consists of a set of sentences, which can be retrieved and modified; a namespace provides a mapping from names to its subcomponents and a name resolution mechanism.
%
The only exception is for interpretations which come in many different flavours (enumerated, symbolic, procedurally interpreted) and can be very large, so a naive enumeration would consume too much memory while access would be inefficient.
%
%An interpretation consists of four table-objects, respectively the ct, cf, pt and pf interpretations of the symbol.
%A table object should be able to check whether it contains certain other objects and should be able to iterate over its contents.
%Strings and domain elements are interned, translation is hashed, containers in grounder instead of explicit substitution

==> 3d-procedural.tex <==
\subsection{Procedural Integration}\label{sec:procedural}
The integration of logic with a procedural language works in two directions.
Within a procedural program, logical components and inferences are available to obtain more complex functionality.
Within a declarative specification, symbols can be interpreted as the result of procedural calls, useful, e.g., for integration with external sources. 

In the former direction, logical objects are made available to a procedural language. For that purpose, \idp allows users to write ``procedure'' components within namespaces that define Lua functions.
%
For example the code \il{procedure append(left, right)\{ return left..right; \};} defines a function ``append'' that takes two arguments and returns their concatenation (``..'' is the string concatenation operator in Lua).
Each logic object and namespace declared in the global namespace is associated with a corresponding object in the Lua run-time environment, with the same name.
%For each logic object in a specification a Lua variable is initialised with the same name and assigned to that object.
Hence, logic object and namespaces are first-class citizens in the Lua stack.
%The data model is built in such a way (using nested tables\footnote{A \emph{table} --which is in fact a dictionary-- is the main datastructure in Lua.}) that logic components can be referred to by their FQN (e.g., the global namespace is available everywhere through the global variable \il{global}).
%
Additionally, \idp inferences and functionalities and ``procedure'' components are available as native Lua functions. 
For example, the code \il{procedure onemodel() \{ return modelexpand(T,S)[1]; \};} will pass the variables \il{T} and \il{S} to the model expansion inference. If these refer to a theory, respectively structure, in the global namespace, model expansion is executed and the first model is returned\footnote{If no models exist,  \il{nil} is returned, the Lua equivalent of an empty reference.}.

In the latter direction (interpreting logical symbols through procedural calls), in a structure, symbols can be interpreted by procedures as follows.
In the context of a structure \I, one can specify the interpretation of a
predicate symbol \il{P[T1...Tn)]} by a Lua boolean function \il{f} with the same
type of arguments as \il{P = procedure f}.
In that case, \il{P(d1...dn)} is true (false) iff \il{f(d1...dn)} returns ``true'', respectively ``false''.
For a function symbol \il{f}, a procedure should, given \il{d1...dn} as input, return the interpretation of \il{f(d1...dn)}, or \il{nil} if the term is non-denoting. For example, interpreting a function by string concatenation, an operation that already exists in Lua, can be modelled as:
\begin{lstlisting}
vocabulary V is { func add[string,string->string]; 
				  func c[->string] }
theory T over V is { c = add("Hello, ", "world.") }
structure S over V is { add = procedure append }
procedure append(left,right) is { return left..right }
\end{lstlisting}
%Or a procedure is provided which returns a Lua iterator, allowing to iterate over the contents of the table in the form of an iterator that returns all matching tuples. Such a procedural interpretation of symbols can serve for easily keeping complex computations out of the logic and also increases the modularity of the system.

Two restrictions on using a Lua function \il{f} as interpretation of a symbol $s$ are (i) that \il{f} is a \emph{pure} function (i.e., the return value should only depend on the input arguments and there should be no side-effects) and (ii) that it results in a consistent interpretation for $s$ that also obeys its type signature.
%The latter assumption can be disabled, but disabling it leads to a possibly expensive check.


\paragraph{\fodot datamodel for Lua.}
An \idp specification organizes its logic components in a hierarchy of namespaces with the namespace $global$ at the root. Referencing a concrete element in this hierarchy is done through \il{n[s]}, with \il{n} the name of a variable that refers to a namespace $N$ and \il{s} the name of a logical object, namespace or procedure that belongs to $N$.
In a similar fashion, an access \il{V[n]}, retrieves the symbol with name \il{n} from vocabulary \il{V}, and \il{S[s]} retrieves the interpretation of the symbol \il{s} from structure \il{S}.

For example, calling the procedure \il{main()} first passes the values of the variables \il{T} and \il{S} to the function \il{onemodel}. Next, the symbol $c$ with name \il{n} is retrieved from the vocabulary \il{V} and is used to retrieve the interpretation of $c$ from the model found. Finally, this interpretation is printed. 
\begin{lstlisting}
procedure main() { print(onemodel(T,S)[V[c]]); }
\end{lstlisting}
\todo{rvwr4: If this is a usual main function, it's not clear where the values of
the variables T, S and V come from.  One would assume they would be
retrieved from the logic component using n[s], v[n], etc. notation?
It would be easier to understand if it were self-contained (or if it
is, how to understand where the variable values come from.)  Could I
use a constant in place of the variable? E.g., database[course] (or
however a constant is written in Lua.)  I'm not clear how you get from
the name of the namespace to the namespace object.  Don't you have to
start at some point with a constant that refers to the namespace to
start with?  I think I'm confused.  Does "global" fix this?  This
paragraph could be made clearer.}

As is often the case, many inferences can be customized in some way.
For example, how structures should be printed (interpretations of sets or lists of facts), how many models a call to model expansion should (try to) return or how much output should be printed while solving a query, \ldots
In \idp, most of these options are set globally through the \il{stdoptions} Lua table.
For example, \il{stdoptions.nbmodels=n;} indicates that subsequent model generation tasks should try to find \il{n} models.


\paragraph{Dynamics.}
Execution of the procedural program requires semantics for the state of logic components at different points in time.
For a component $C$, we refer to its ``version'' at time $t$ as $C_t$, with $C_1$ that state after parsing.
Datamodel operations change the underlying logic components (not just the contents of Lua variables).
Dependencies in the declarative component of the language, such as includes, are \emph{dynamic}.
E.g., if a vocabulary $V$ includes vocabulary $V'$ and at $t$, a new symbol $P$ is added to $V'$, then $V_{t+1}$ also contains $P$.
A similar principle holds for structures, theories, \ldots

Such a behaviour is required to support modularity during execution. For example, consider a robot adding knowledge to his \il{world} theory that contains basic knowledge about the world around him.
One would expect any theory including \il{world} to automatically refer to the newest knowledge instead of to a copy of the old information.

\todo{Voorbeeld van dynamics.}

\paragraph{File inclusion.}
The main method of creating logic objects is through providing a list of files, which are then parsed into the relevant logic objects.
To allow distributing knowledge over multiple files, the \emph{require} statement is provided: a file that contains a statement \il{require file;} instructs \idp to also load the file \il{file}. For example, one can construct a file with a structure for each instance of a problem and this file can require to load the file(s) containing the vocabularies, the theories, the task, etc., needed to solve the problem of which the structure is an instance. It then suffices to load a single file to solve an instance.
%
The system provides built-in packages with general-purpose components. These include predefined vocabularies and theories as well as extra inference methods, and can be included through \il{require-std name}, with \il{name} the name of the package. For example, \il{require-std mx} includes useful procedures related to model expansion. %Built-in components are typically part of the namespace \il{stdspace}.


\paragraph{Interactive shell.}
Both Lua and \fodotidp are interpreted languages (or, at least, compiled Just-In-Time).
This allows \idp to provide an interactive interpreter for the language, similar to interpreters available in, e.g., many Prolog systems, by executing Lua code on the fly.
The interpreter provides \emph{autocompletion}, suggesting available \idp procedures that match a partial input; the autocompletion also specifies the expected argument types. 
Files can be loaded dynamically through \il{loaddependency(file)}.


==> idp-latex/idp-latex-no-theorem.tex <==
%IMPORTANT: ONLY INCLUDE AS \input{idp-latex/idp-latex-no-theorem}
\usepackage{import}

\subimport{idp-latex/}{includes-no-theorems}
\subimport{idp-latex/}{common-citations}




%The following are directives for LaTeX editors that collect ``included files'' to autocomplete macros etcetera
\ignore{
\include{includes-no-theorems}
\include{common-citations}
}

==> image_mx.tex <==
% Define block styles
\tikzstyle{block} = [draw=red, fill=blue!20, rectangle, rounded corners, inner sep=10pt, inner ysep=20pt]
\tikzstyle{mainblock} = [draw=blue, fill=blue!20, very thick, rectangle, rounded corners, inner sep=10pt, inner sep=8pt]
\tikzstyle{fancytitle} =[fill=NavyBlue, text=white]

\pgfdeclarelayer{background}
\pgfdeclarelayer{foreground}
\pgfsetlayers{background,main,foreground}
    
\begin{figure}
\centering
\begin{tikzpicture}[auto, every text node part/.style={align=left}, node distance = 0.5cm]
\node [mainblock, text width=11.5cm] (knowledge) { 
\begin{lstlisting}[frame=no]
vocabulary V is {
	type day; type hour; type course;
	type time constructed from { time(day,hour) };	
	type session;	type teacher;	type student;		
	courseOf[session -> course];	timeOf[session, time];
	teaches[teacher,course];		takes[student,course];
	teacherOf[session->teacher];	attends[student,session];
	overlaps[session,session];
};
vocabulary Vout is {
	include V::courseOf;   include V::timeOf;
	include V::attends;    include V::teacherOf;

};
theory T over T {
	!s: ?=1 t: timeOf(s,t);
	definition { 
		!s1 s2: overlaps(s1,s2) <-  
                  s1~=s2 & ?t: timeOf(s1,t) & timeOf(s2,t); 
    }

	!s1 s2: overlaps(s1,s2) 
						=> teacherOf(s1)~=teacherOf(s2);
	
	!student sess: attends(student,sess)
						=> takes(student, courseOf(sess));
	...
};
term C over T is // number of conflicts
    #({stud s1 s2: overlaps(s1,s2) & attends(stud,s1) & attends(stud,s2)});
\end{lstlisting}
};

%	!student,course: takes(student,course) 
%		=> ?=1 sess: courseOf(sess)=course & attends(student,sess);
%	replacement(teacher,session);
%	include V::replacement;
%	!sess: (?repl: replacement(repl,sess)) 
%			<=> ~teaches(teacherOf(sess), courseOf(sess));

\node [mainblock, below=of knowledge.south west, text width=5.2cm, anchor = north west] (inferences) {
minimize(T, db, C, Vout)
\begin{enumerate}
	\item Structure consistency check
	\item Detect + exploit functions
	\item Detect + break symmetries
	\item Derive variable bounds
	\item Ground with bounds + search
	\item Post-process definition
\end{enumerate}
};

\node [mainblock, right=of inferences.east] (proceduralint) {
\begin{lstlisting}[frame=no]
procedure solve(db) {
    m = minimize(T,db,C,Vout);
    conf = value(C,m);
    print("Conflicts = "..conf);
    return m;
};
\end{lstlisting}
};
	
\node[fancytitle, right=10pt] at (proceduralint.north west) {Procedure interface};
\node[fancytitle, right=10pt] at (inferences.north west) {Inferences};
\node[fancytitle, right=10pt] at (knowledge.north west) {Knowledge};
\end{tikzpicture}
\caption{A (simplified) example of a course scheduling problem.
For each course, several sessions are organized and each student should attend one session for each course taken.
For each session, a time slot, teacher and list of students have to be found that satisfy constraints such as no teacher nor student overlap and a limited number of students in each session. 
Optimal model expansion is then applied to minimize the number of conflicts for students, through the inference workflow shown on the left.
}
\label{fig:mx}
\end{figure}

==> running_example.tex <==
University course administration

\begin{lstlisting}
vocabulary time{
	type day constructed from { monday, tuesday, wednesday, thursday, friday, saturday, sunday};
	type hour isa nat;
	type time constructed from { moment(day,hour) domain validmoment(day,hour)}; // woensdagnamiddag niet ofzo?
	func day(time):day
	func hour(time):hour
	partial func add(time,time):time
}
theory calendar over time {
	{
		validmoment(d,h) <- h>8 & h<20 & d~=sunday & (if d=wednesday then h<13).
		hour(moment(d,h)=h.
		day(moment(d,h)=d.
		add(moment(d,h),moment(d,h2))=moment(d,h+h2) <- h+h2<24.
		...  // wrapping rules
	}
}
vocabulary database {
	type course;
	type location;
	
	type person;
	type student isa person;	
	type teacher isa person;
	
	pred takes[student,course];
	pred teaches[teacher,course];
	
	include time;	
	
	type session;
	func course[session -> course];
	func length[session -> nat]; // in hours
		
	pred available[teacher, time];
};

vocabulary schedule {
	include database;
	
	func planned[session -> time];
	func planned[session -> location];
	
	pred attends(student, session)
	overlaps(session,session)
};

// Guarantee loop-freeness of course dependencies
theory T over courses {
	define {
		canBeTaken(c) <- !c2: dependsOn(c,c2) => canBeTaken(c2); 
	};
	constraint !c: canBeTaken(c);
};

theory T over schedule {
	constraint available(teaches(course(session)),planned(session));
	define {
		overlaps(s1,s2) <- planned(s1)=<planned(s2)=<add(planned(s1),length(s1)) | overlaps(s2,s1);
	};
	constraint takes(student,course(session)) => attends(student,session);
	
	constraint overlap(s1,s2) => planned[session->location](s1)~=planned[session->location](s2);
};

term nbOfConflicts over schedule {
	#{student: ?s1 s2: s1~=s2 & attends(student,s1) & attend(student,s2) & overlaps(s1,s2)}
}

structure S over database {
	available = procedure checkExternalCalendar
};

procedure checkExternalCalendar(teacher, time){
	
}

theory print over schedule {
	{
		output(append/sort()).?
	}
}

\end{lstlisting}
